Algorithms for a Topology-aware Massively Parallel Computation Model

Most of the prior work in massively parallel data processing assumes homogeneity, i.e., every computing unit has the same computational capability, and can communicate with every other unit with the same latency and bandwidth. However, this strong assumption of a uniform topology rarely holds in practical settings, where computing units are connected through complex networks. To address this issue, Blanas et al. recently proposed a topology-aware massively parallel computation model that integrates the network structure and heterogeneity in the modeling cost. The network is modeled as a directed graph, where each edge is associated with a cost function that depends on the data transferred between the two endpoints. The computation proceeds in synchronous rounds, and the cost of each round is measured as the maximum cost over all the edges in the network. In this work, we take the first step into investigating three fundamental data processing tasks in this topology-aware parallel model: set intersection, cartesian product, and sorting. We focus on network topologies that are tree topologies, and present both lower bounds, as well as (asymptotically) matching upper bounds. The optimality of our algorithms is with respect to the initial data distribution among the network nodes, instead of assuming worst-case distribution as in previous results. Apart from the theoretical optimality of our results, our protocols are simple, use a constant number of rounds, and we believe can be implemented in practical settings as well.

==> asymmetric.tex <==
\section{Asymmetric Star}

In this section, we turn to the asymmetric nework by considering set intersection on the star topology. We first consider two simple versions as warm-up: sending-free star with $w(v,o) = \infty$ for any $v \in V_C$, and receiving-free star with $w(o,v) = \infty$ for any $v \in V_C$, where $o$ is the center node. Then, we extend both cases to a general asymmetric star.

A primitive argument that commonly used in deriving the lower bound is as follows. Consider an arbitrary edge $e = (o,v)$. Denote the amount of data sent from $v$ to $o$ as $x$, and that from $o$ to $v$ as $y$. There must be: (1) if $y < \min\{|R|-|R_v|,|S|-|S_v|\}$, then $x \ge N_v$; (2) if $\min\{|R| - |R_v|, |S| - |S_v|\} \le y < \max\{|R| - |R_v|, |S| - |S_v|\}$, then $x \ge |R_v|$ if $|R| - |R_v| < |S| - |S_v|$ and $x \ge |S_v|$ otherwise;  (3) if $x < \min\{|R_v|,|S_v|\}$, then $y \ge N- N_v$; (4) if $\min\{|R_v|, |S_v|\} \le x < \max\{|R_v|, |S_v|\}$, then $y \ge |S|-|S_v|$ if $|R_v| > |S_v|$ and $y \ge |R|-|R_v|$ otherwise. These observations are directly implied by the Alice-Bob communication model. For simplicity,   assume $|R| \le |S|$. 


\subsection{Sending-free Star} 
Assume $w(o,v) = \infty$ for any compute node $v \in V_C$.For simplicity, denote $W = \sum_{v \in V_C} w_v$. We first introduce the hash join on the sending-free star. This version of HJ algorithm is named as {\em sfHJ}. Similarly, by designing a set of hash functions, each node $v \in V_C$ sends its local data to node $u$ with probability $p_u$, where $p_u = w_u /W$. The expected amount of data sent to node $u$ is bounded by $\sum_{v: v \neq u} \cdot w_u /W$, which incurs a capacity cost of $O(\frac{N}{W})$. 

Let $C_{opt}$ be the optimal cost of any algorithm correctly computing $R \cap S$.

\begin{lemma}
	\label{lem:lb-send-free-star}
	The following lower bound holds
	\begin{align*}
		C_{opt} \ge \min_{(V_\alpha, V_\beta)} &\max\{\max_{v \notin V_\alpha} \frac{|S| - |S_v|}{w_v}, \max_{v \notin V_\beta} \frac{|R| - |R_v|}{w_v}\} + \frac{1}{W} \cdot (\sum_{v \in V_\alpha} |R_v| + \sum_{v \in V_\beta} |S_v|) 
	\end{align*}
	where $V_\alpha, V_\beta$ is over all subsets of $V_C$ satisfying the property: if $V_C - V_\alpha \neq \emptyset$ and $V_C - V_\beta \neq \emptyset$, then $V_\alpha = V_\beta$ and $|V_\alpha| = |V_\beta| = |V_C| -1$.
\end{lemma}

\begin{proof}
	Consider an algorithm correctly computing $R \cap S$ with capacity cost $C$.
	In the computation, the compute nodes in $V_C$ can be divided into two subsets, $V_\alpha$ including those sending out their $R$-tuples and $V_\beta$ including those sending out their $S$-tuples. 
	
	The constraint on $V_\alpha, V_\beta$ guarantees the correctness of the algorithm. By contradiction, assume  $u \in V_C - V_\alpha, v \in V_C - V_\beta$ for $u \neq v$. Then at least one  $R$-tuples does not leave $u$ and at least one $S$-tuple does not leave $v$, thus no way to compute $R_u \cap S_v$, coming to a contradiction. 
	
	Consider a compute node $v$. If $v \notin V_\alpha$, at least one tuple in $R_v$ does not leave $v$. In order to guarantee the correctness, all data in $S-S_v$ must be sent to node $v$, hence $C \ge (|S| - |S_v|)/w_v$. Thus, $C \ge \max_{v \neq V_\alpha} (|S| - |S_v|)/w_v$. Using a symmetric argument, $C \ge \max_{v \neq \beta} (|R|-|R_v|)/w_v$. Moreover, the tuples sent out by nodes in $V_\alpha \cup V_\beta$ will be distributed to at least one node, hence $C \cdot W \ge \sum_{v \in V_\alpha} |R_v| + \sum_{v \in V_\beta} |S_v|$. The lower bound takes the minimum capacity cost over all correct algorithms, i.e., all choices of $(V_\alpha, V_\beta)$, resulting in the formula in Lemma~\ref{lem:lb-send-free-star} as desired.
\end{proof}


Our algorithm is described in {\sc SFStarIntersect}. It picks the best of three strategies. The capacity of the first strategy is $C_1 = \min_v (N - N_v)/w_v$.

\begin{algorithm}[h]
	\caption{{\sc SFStartIntersect}$(G, \dstr)$}
	\label{alg:intersect-send-free-star}
	
	Pick the best out of:
	\begin{packed_enum}
		\item	All compute nodes send its data to $\arg \min_v \frac{N-N_v}{w_v}$\;
		
		\item $V_1 = \{v \in V_C: |R| - |R_v| > |S| - |S_v|\}$\;
		$V^*_1 = \arg \min L(V_1, \frac{|S| - |S_v|}{w_v}, \frac{|R_v|}{W})$\;
		All compute nodes send their $S$-tuples to nodes in $V^*_1$\;
		Invoke the sfHJ on the star to compute $(\bigcup_{v \notin V^*_1} R_v) \cap S$\;
		
		\item $V_2 = \{v \in V_C: |R| - |R_v| \le |S| - |S_v|\}$\;
		$V^*_2 = \arg \min L(V_2, \frac{|R| - |R_v|}{w_v}, \frac{|S_v|}{W})$\;
		All compute nodes send their $R$-tuples to nodes in $V^*_2$\;
		Invoke the sfHJ on the star to compute $R \cap (\bigcup_{v \notin V^*_2} S_v)$\;
		
	\end{packed_enum}
\end{algorithm}

Before introducing the second and third strategy, we first introduce an optimization problem as below:
\[\min_{X \subseteq V} \max_{v \in X} f(v) + \sum_{v \notin X} g(v)\]
where $V$ is a set of elements and $f, g$ are two functions defined on $V$. The optimal solution is denoted as $L(V, f, g)$. Observe that it is possible to compute $L(V, f, g)$ in time of $O(|V_C|)$.
In this way, define $V^*_1 = \arg \min L(V_1, \frac{|S| - |S_v|}{w_v}, \frac{|R_v|}{W})$ and $V^*_2 = \arg \min L(V_2, \frac{|R| - |R_v|}{w_v}, \frac{|S_v|}{W})$, where 
\begin{align*}
	V_1 &= \{v \in V_C: |R| - |R_v| > |S| - |S_v|\} \\
	V_2 &= \{v \in V_C: |R| - |R_v| \le |S| - |S_v|\}
\end{align*} 

In the second strategy, each node in $V^*_1$ receives all data in $S - S_v$ and then computes $R_v \cap S$. Then it invokes the sfHJ algorithm to compute $(\bigcup_{v \notin V^*_1} R_v) \cap S$. Its capacity cost is thus 
\begin{align*}
	 C_2 =  & \max_{v \in V^*_1} \frac{|S| - |S_v|}{w_v} + \frac{|S|}{W} + \sum_{v \notin V^*_1} \frac{|R_v|}{W}\\
	 = & L(V_1, \frac{|S| - |S_v|}{w_v}, \frac{|R_v|}{W}) + \frac{|S|}{W} + \sum_{v \in V_2} \frac{|R_v|}{W} 
\end{align*} 

The third strategy is symmetric with the second one. Each node in $V^*_2$ receives all data in $R - R_v$ and then computes $R \cap S_v$. Then it invokes the sfHJ algorithm to compute $R \cap (\bigcup_{v \notin V^*_2} S_v)$. Its capacity cost is thus 
\begin{align*}
	C_3 = L(V_2, \frac{|R| - |R_v|}{w_v}, \frac{|S_v|}{W}) + \frac{|R|}{W} + \sum_{v \in V_1} \frac{|S_v|}{W}
\end{align*} 

Taking the min of the three cases, this algorithm has a capacity cost of $C_{alg} = \min\{C_1, C_2, C_3\}$. Lemma~\ref{lem:optimality-send-free-star} tells us that $C_{alg} \le \copt$, thus proving the optimality of this algorithm.

\begin{lemma}
	\label{lem:optimality-send-free-star}
	$C_{opt} \ge C_{UB}$.
\end{lemma}

\begin{proof}
	Implied by the property of $(V_\alpha, V_\beta)$, we consider three cases of the $(V_\alpha, V_\beta)$ as below.
	
	\paragraph{Case 1: $V_C - V_\alpha \neq \emptyset$ and $V_C - V_\beta = \emptyset$} Note that only one node exists in $V_C - V_\alpha$ or $V_C - V_\beta$. The lower bound can be rewritten as 
	\[C_{opt} \ge \min_v \frac{N-N_v}{w_v} + \frac{1}{W} (N-N_v) \ge C_1\]
	which is a contradiction to $C_{opt} < \min_v (N - N_v)/w_v$. 
	
	\paragraph{Case 2: $V_C - V_\alpha = \emptyset$} The lower bound becomes 
	\begin{align*}
	C_{opt} \ge  \frac{|R|}{W}  + \min_{V_\beta} (\max_{v \notin V_\beta} \frac{|R| - |R_v|}{w_v} + \sum_{v \in V_\beta} \frac{|S_v|}{W})
	\end{align*}
	Observe that for node $v \in V_1$, there is $v \in V_\beta$; otherwise, $C_{opt} \cdot w_v > |R| - |R_v|\ge \frac{1}{2}(N - N_v)$, coming to a contradiction. Denote $\hat{V}_\beta = V_C - V_\beta$. We reformulate the lower bound as
	\begin{align*}
	C_{opt} & \ge \frac{|R|}{W}  + \sum_{v \in V_1} \frac{|S_v|}{W} +  \min_{\hat{V}_\beta \subseteq V_2} (\max_{v \in \hat{V}_\beta} \frac{|R| - |R_v|}{w_v} +  \sum_{v \in V_2 - \hat{V}_\beta} \frac{|S_v|}{W})\\
	& \ge \frac{|R|}{W}  + \sum_{v \in V_1} \frac{|S_v|}{W} +  L(V_2, \frac{|R| - |R_v|}{w_v}, \frac{|S_v|}{W})  = C_3   
	\end{align*}
	
	\paragraph{Case 3: $V_C - V_\beta = \emptyset$} Using a symmetric argument, the lower bound in this case becomes 
	\begin{align*}
	C_{opt}  \ge \frac{|S|}{W}  + \sum_{v \in V_2} \frac{|R_v|}{W} +  L(V_1, \frac{|S| - |S_v|}{w_v}, \frac{|R_v|}{W}) = C_2
	\end{align*}
	
	Over all cases, we have shown that $C_{opt} \ge C_{UB}$.

\end{proof}



\begin{lemma}
	On a sending-free asymmetric star topology, {\sc SFStarIntersect} computes the intersection $R \cap S$ with cost $O(\log N)$ away from the optimal solution.
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Receiving-free Star}
Assume $w(v,o) = \infty$ for any compute node $v \in V_C$.
In this case, we want to minimize the maximum cost of sending data out of each compute node.

\begin{lemma} \label{lem:lb-receive star}
Let $C_{opt}$ be the optimal cost of an algorithm that computes set intersection on a receiving-free star topology. Then,
$C_{opt} \ge \max_v L^{\mathsf{rf}}(v)$, where
\[L^{\mathsf{rf}}(v) = \max \left\{ \min\{\frac{|R_v|}{w_v}, \max_{u \neq v} \frac{|S_u|}{w_u}\}, \min\{\frac{|S_v|}{w_v}, \max_{u \neq v} \frac{|R_u|}{w_u}\} \right\} \]
\end{lemma}

\begin{proof}
Suppose that for some $v$ that there exists an algorithm (w.l.o.g.) with cost
$C <  \min\{\frac{|R_v|}{w_v}, \max_{u \neq v} \frac{|S_u|}{w_u}\}$. We will show how to use this
protocol to beat the lopsided communication complexity lower bound.
Let Alice hold $|R_v|$ data, and Bob $|S_u|$, where $u  = \arg\max_{i \neq v} |S_i|/w_i$. To compute the set intersection, we can
use the algorithm on receiving star as follows: Alice sits at node $v$, Bob at node $u$, and the rest of the data
that is not $R_v,S_u$ can be padded with disjoint data that will not intersect. 
Then, to compute $R \cap S$, Alice cannot send more than $ |R_v|$ bits and Bob cannot send more than $|S_u|$ bits,
contradicting the lower bound. 
%Consider a compute node $v \in V_C$ that holds $R_v, S_v$. Suppose $C_{opt} < |R_v|/w_v$. Then at least one tuple in $R_v$ does not leave node $v$, in order to guarantee the correctness, all data in $S - S_v$ must be sent to node $v$, i.e., for any node $u \neq v$, every $S$-tuple in $S_u$ must be sent out to the router, hence $C_{opt} \ge \max_{u \neq v}|S_u|/w_u$. Thus, $C_{opt} \ge \min\{|R_v|/w_v, \max_{u \neq v} |S_u|/w_u\}$. Using a symmetric argument, $C_{opt} \ge \min\{|S_v|/w_v, \max_{u \neq v} |R_u|/w_u\}$. Summing up the two inequalities, we can obtain the desired result.
\end{proof}



\introparagraph{Algorithm} The algorithm simply chooses the best out of the following three deterministic strategies:
	\begin{packed_enum}
	\item	Each compute node sends its data to $\arg \max_v \frac{N_v}{w_v}$\;
	\item Each compute node	broadcasts the $R$-tuples \;
	\item Each compute node broadcasts the $S$-tuples \;		
	\end{packed_enum}


\begin{lemma}
On a receiving-free asymmetric star topology, we can compute the intersection $R \cap S$ with cost $O(\log N)$ away from the optimal solution.
\end{lemma}

\begin{proof}
Let $\twomax$ denote the second largest value of a set. Then, the capacity cost of the above algorithm (measured in tuples) is: 
%
\[C_{alg} = \min\{\twomax_v \frac{N_v}{w_v}, \max_v \frac{|R_v|}{w_v}, \max_v \frac{|S_v|}{w_v}\}\]
Lemma~\ref{lem:optimality-intersect-receive-free-star} (proved in the appendix) tells us that $C_{alg} \leq \max_v L^{\mathsf{rf}}(v)$, thus proving the claim.
\end{proof}

\begin{lemma}
	\label{lem:optimality-intersect-receive-free-star}
	$ \min\{\twomax_v \frac{N_v}{w_v}, \max_v \frac{|R_v|}{w_v}, \max_v \frac{|S_v|}{w_v}\} \leq 2 \max_v \max \left\{ \min\{\frac{|R_v|}{w_v}, \max_{u \neq v} \frac{|S_u|}{w_u}\}, \min\{\frac{|S_v|}{w_v}, \max_{u \neq v} \frac{|R_u|}{w_u}\} \right\}$.
\end{lemma}

\begin{proof}
	Let $i = \arg \max_{u} |R_u|/w_u$ and $j = \arg \max_{u} |S_u|/w_u$.
	We distinguish two cases.
	
	\paragraph{Case 1: $i \neq j$} Then, $LHS \leq \min\{ \frac{|R_i|}{w_i},  \frac{|S_j|}{w_j}\}$.
	As for the right-hand side, 
	%
	\[ RHS \geq 2 \min\{\frac{|R_i|}{w_i}, \max_{u \neq i} \frac{|S_u|}{w_u}\}  = 2 \min\{\frac{|R_i|}{w_i}, \frac{|S_j|}{w_j}\} \]
	
	\paragraph{Case 2: $i = j$} For the right-hand side, we have:
	\[ RHS \geq 2 \max  \left\{ \min\{\frac{|R_i|}{w_i}, \twomax \frac{|S_u|}{w_u}\} , \min\{\frac{|S_i|}{w_i}, \twomax \frac{|R_u|}{w_u}\} \right\} \]
	The inequality is straightforward if $\frac{|R_i|}{w_i} < \twomax \frac{|S_u|}{w_u}$ or $\frac{|S_i|}{w_i} < \twomax \frac{|R_u|}{w_u}$.
	If not, the right-hand side becomes: 
	\[ RHS \geq 2 \max  \left\{ \twomax \frac{|S_u|}{w_u},  \twomax \frac{|R_u|}{w_u} \right\} 
	\geq  \twomax \frac{|S_u|}{w_u} + \twomax \frac{|R_u|}{w_u} \geq \twomax_v \frac{N_v}{w_v} \]
	where the last inequality follows from the fact that $i$ maximizes both ratios. 
\end{proof}


\subsection{General Asymmetric Star}

Let $C_{opt}$ be the capacity cost of any algorithm correctly computing $R \cap S$.  The following lower bound is a generalization of both Lemma~\ref{lem:lb-send-free-star} and Lemma~\ref{lem:lb-receive star}.

\begin{lemma}
	\label{lem:lb-intersect-asym-star}
	The following lower bound holds:
	\begin{displaymath}
	 C_{opt} \ge	\min_{V_\alpha, V_\beta} \max \left\{ \begin{array}{ll}
	\max_{v \in V_\alpha} |R_v|/w_{vo} \\
	\max_{v \notin V_\alpha} \max\{\frac{|S| - |S_v|}{w_{ov}},  \max_{u \neq v} \frac{|S_u|}{w_{uo}}\} \\
	\max_{v \in V_\beta} |S_v|/w_{vo} \\
	\max_{v \notin V_\beta} \max\{\frac{|R| - |R_v|}{w_{ov}},  \max_{u \neq v} \frac{|R_u|}{w_{uo}} \} \\
	(\sum_{v \in V_\alpha} |R_v| + \sum_{v \in V_\beta} |S_v|) /\sum_{v} w_{ov}
	\end{array} \right.
	\end{displaymath}
	where $V_\alpha, V_\beta$ over all subsets of $V_C$ satisfying the following properties: If $V_\alpha \subsetneq V_C$ and $V_\beta \subsetneq V_C$, then $V_\alpha = V_\beta$ and $|V_\alpha| = |V_\beta| = |V_C| -1$.
\end{lemma}

\begin{proof}
	Consider an algorithm correctly computing $R \cap S$ with capacity cost $C$.
	In the computation, the compute nodes in $V_C$ can be characterized by two subsets, %%$V_\alpha$ including those receiving all data of $S-S_v$, 
	$V_\alpha$ including those sending out all of their $R$-tuples, %%$V_\gamma$ including those receiving all data of $R - R_v$, 
	and $V_\beta$ including those sending out all of their $S$-tuples.

	For any node $v \in V_\alpha$, at least one tuple in $R_v$ does not leave $v$. In order to guarantee the correctness, all data in $S -S_v$ must be sent to $v$. Using a symmetric argument, for any node $v \in V_\gamma$, all data in $R -R_v$ must be sent to $v$.
	As the $R$-tuples sent out by nodes in $V_\alpha$ and the $S$-tuples sent out by nodes in $V_\beta$ will be distributed to at least one node, thus $C \cdot \sum_v w_{ov} \ge \sum_{v \in V_\alpha} |R_v| + \sum_{v \in V_\beta} |S_v|$.  Together, we can obtain all contraints on $C$.
	
	For the contraint on $V_\alpha, V_\beta$, assume $u \in V_C - V_\alpha$ and $v \in V_C - V_\beta$ for $u \neq v$ by contradiction. Observe that at least one tuple of $R_u$ does not leave $u$ and at least one tuple of $S_v$ does not leave $v$, thus no way to compute $R_u \cap S_v$, coming to a contradiction.
	
	Taking the minimum cost over all correct algorithms, we will get  the formula in Lemma~\ref{lem:lb-intersect-asym-star} as desired.
\end{proof}


\begin{algorithm}[h]
	\caption{{\sc AsymStartIntersect}$(G, \dstr)$}
	\label{alg:intersect-asym-star}
	Pick the best out of:
	\begin{packed_enum}
		\item	All compute nodes send their data to $\arg \min_v \max\{\frac{N-N_v}{w_{ov}}, \max_{u \neq v} \frac{N_u}{w_{uo}}\}$\;
		
		\item $V^*_1 = \arg \min L(V_C, \frac{|S| - |S_v|}{w_{vo}}, \frac{|R_v|}{w_{vo}}, \frac{|R_v|}{\sum_v w_{ov}})$\;
		All comute nodes send their $S$-tuples to node in $V^*_1$\;
		Invoke the swHJ alogrithm on the star to compute $(\bigcup_{v \notin V^*_1} R_v) \cap S$.
		
		\item $V^*_2 = \arg \min L(V_C, \frac{|R| - |R_v|}{w_{vo}}, \frac{|S_v|}{w_{vo}}, \frac{|S_v|}{\sum_v w_{ov}})$\;
		All comute nodes send their $R$-tuples to node in $V^*_2$\;
		Invoke the swHJ alogrithm on the star to compute $R \cap (\bigcup_{v \notin V^*_2} S_v)$.
	\end{packed_enum}
\end{algorithm}

Our algorithm is described in {\sc AsymStartIntersect}. It picks the best out of three strategies and the correctness is clear. The capacity cost of the first strategy is
\begin{align*}
	C_1 = \min_v \max\{\frac{N-N_v}{w_{ov}}, \max_{u \neq v} \frac{N_u}{w_{uo}}\} 
\end{align*}

Before introducing the second and third strategy, we introduce the following optimization problem:
\[\min_{X \subseteq V} \max_{v \in X} f(v) + \max_{v \notin X} g(v) + \sum_{v \notin X} h(v)\]
where $V$ is a set of elements, and $f, g, h$ are three functions defined on $V$. The optimal solution is denoted as $L(V, f, g, h)$. Observe that it is possible to compute $L(V,f,g,h)$ in time $O(|V_C|)$. Define 
\begin{align*}
	V^*_1 = & \arg \min L(V_C, \frac{|S| - |S_v|}{w_{vo}}, \frac{|R_v|}{w_{vo}}, \frac{|R_v|}{\sum_v w_{ov}}) \\
	V^*_2 = & \arg \min L(V_C, \frac{|R| - |R_v|}{w_{vo}}, \frac{|S_v|}{w_{vo}}, \frac{|S_v|}{\sum_v w_{ov}})
\end{align*}
The capacity cost of the second strategy is characterized by 
\begin{align*}
	C_2 =  \max\{ & \max_{v} \frac{|S_v|}{w_{vo}} +  \max_{v \notin V^*_1} \frac{|R_v|}{w_{vo}},  \max_{v \in V^*_1} \frac{|S| - |S_v|}{w_{ov}} +   \frac{1}{\sum_{v} w_{ov}}( |S| + \max_{v \notin V^*_1} |R_v|) \}
\end{align*}
Symmetrically, the capacity of the thrid strategy is 
\begin{align*}
	C_3 =  \max\{ & \max_{v} \frac{|R_v|}{w_{vo}} +  \max_{v \notin V^*_2} \frac{|S_v|}{w_{vo}},  \max_{v \in V^*_2} \frac{|R| - |R_v|}{w_{ov}} +   \frac{1}{\sum_{v} w_{ov}}( |R| + \max_{v \notin V^*_2} |S_v|) \}
\end{align*}
The capacity cost of Algorithm~\ref{alg:intersect-asym-star} is $C_{alg} = \min\{C_1, C_2, C_3\}$. Lemma~\ref{lem:optimality-intersect-asym-star} tells us that $C_{alg} \le \copt$, thus this algorithm is optimal.

\begin{lemma}
	\label{lem:optimality-intersect-asym-star}
	$C_{opt} \ge C_{alg}$.
\end{lemma}

\begin{proof}
	It suffices to show that $C_{opt} \ge \min\{C_2, C_3\}$ under the condition that $C_{opt} <  C_1$.
	Consider the three cases.
	
	\paragraph{Case 1: $V_C - V_\alpha \neq \emptyset$ and $V_C - V_\beta \neq \emptyset$} By our analysis above, there is one node in $(V_C - V_\alpha) \cap (V_C - V_\beta)$, w.l.o.g. assume $V_C - V_\alpha - V_\beta = \{v^*\}$. 
	There must be \[C_{opt} \ge \max\{ \frac{N-N_v^*}{w_{ov^*}}, \max_{v \neq v^*} \frac{N_v}{w_{vo}}\}\]
	which is a contradiction to the fact that $C_{opt} < \max\{(N - N_v)/w_{ov}, \max_{u \neq v} N_u/w_{uo}\}$ for every $v \in V_C$. 
	
	\paragraph{Case 2: $V_C - V_\beta = \emptyset$} In this case, $C_{opt} \ge |S_v|/w_{vo}$ for every node $v \in V_C$ and the lower bound becomes
	\begin{displaymath}
	C_{opt} \ge \min_{V_\alpha} \max \left\{ \begin{array}{ll}
	\max_{v \notin V_\alpha} (|S| - |S_v|)/w_{ov} \\
	\max_{v \in V_\alpha} |R_v|/w_{vo} \\
	\max_{v} |S_v|/w_{vo} \\
	(\sum_{v \in V_\alpha} |R_v| + \sum_{v} |S_v|) /\sum_{v} w_{ov}
	\end{array} \right.
	\end{displaymath}
	The lower bound can be rewritten as
	\begin{align*}
	C_{opt} \ge & \frac{1}{4} (\max_v \frac{|S_v|}{w_{vo}} + \frac{|S|}{\sum_{v} w_{ov}}) +   \frac{1}{4} \min_{V_\alpha} \max\{	\max_{v \notin V_\alpha} \frac{|S| - |S_v|}{w_{ov}}, \max_{v \in V_\alpha} \frac{|R_v|}{w_{vo}}, \sum_{v \in V_\alpha} \frac{|R_v|}{\sum_v w_{ov}} \} \\
	\ge & \frac{1}{4}  (\max_v \frac{|S_v|}{w_{vo}} +   \frac{|S|}{\sum_{v} w_{ov}}) + \frac{1}{4}  L(V_C, \frac{|S| - |S_v|}{w_{vo}}, \frac{|R_v|}{w_{vo}}, \frac{|R_v|}{\sum_v w_{ov}})
	\end{align*}
	
	\paragraph{Case 3: $V_C - V_\alpha = \emptyset$} It is symmetric with Case 3. The lower bound is at least \begin{align*}
	C_{opt} \ge &  \frac{1}{4} (\max_v \frac{|R_v|}{w_{vo}} + \frac{|R|}{\sum_{v} w_{ov}}) + \frac{1}{4}L(V_C, \frac{|R| - |R_v|}{w_{vo}}, \frac{|S_v|}{w_{vo}}, \frac{|S_v|}{\sum_v w_{ov}})
	\end{align*}
	
	As $C_{opt}$ must fall into any one of the three cases, there is $C_{opt} \ge \min\{C_2, C_3\}$ under the condition that $C_{opt} < C_1$.
\end{proof}


==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

Historically CPU performance increased by raising clock frequencies---a phenomenon referred to as Dennard scaling. About ten years ago, the breakdown of Dennard scaling rekindled interest in parallel data processing and gave rise to new parallel processing frameworks such as MapReduce and Spark. In this setting, the algorithmic complexity of a data processing algorithm is no longer dominated by the number of CPU instructions or disk accesses, but by communication.

One popular theoretical model for studying massively parallel data processing algorithms is the Massively Parallel Computation (MPC) model~\cite{beame:communication}. In the MPC model, any pair of compute nodes communicate via a public point-to-point channel. In each round, all nodes exchanges messages and then perform local computation. The complexity of an algorithm in MPC is measured by the number of rounds and the ``load'' of the nodes, where the load is defined as the maximum size of all messages received by a node in a round.

As the data volume continues to increase, this necessitates ever-larger clusters for data processing. Today one can rent many thousands of CPU cores from cloud vendors for a few hundred dollars per hour. A critical shortcoming of the MPC model for modeling such large clusters is that it is oblivious to the topology of the network. Specifically, the MPC model assumes that any pair of nodes can communicate at the same speed. However, large deployments, such as in the cloud, offer different bandwidths between nodes within the same rack, across racks and across datacenters. Furthermore, in addition to static effects from the network topology, a model needs to capture dynamic effects of different algorithms that can cause contention in the network.

Recent work has started taking into account the impact of network topology for specific problems, such as k-party communication \cite{chattopadhyay2014topology, chattopadhyay2017tight} and aggregation \cite{langberg2019topology}. However, this prior work stops short of introducing a general model that one can use to reason about the complexity of relational data processing algorithms at large scale. %\spyros{Pari, the previous sentences need some work to highlight the contrast with prior work, esp. [11] which is also a PODS paper.}

This paper introduces a new parallel data processing model that is cognizant of the network topology when determining the cost of communication for common data processing algorithms.
We describe the network as a directed graph, where each edge is associated with a cost function that depends on the data transferred between the two endpoints. The computation proceeds in rounds, and the cost of each round is measured as the maximum cost over all the edges in the network. Our proposed model is general enough to capture the MPC model as a special case.


The new network-aware model is used to study three ubiquitous data processing algorithms, namely set intersection, cartesian product and join, which are the building blocks for more complicated analytical queries in database systems. Prior complexity results assume the worst-case or uniform initial data distribution. We study algorithms in a more fine-grained manner by assuming that the initial data cardinality distribution is known in advance. Obviously, if an algorithm is optimal under some initial data cardinality distribution, then it must be optimal in either worst-case or uniform distribution. We assume that cardinality distribution information on the base tables is known from statistics and can be approximately estimated for intermediate results.

Although the model can capture arbitrary network topologies, computer networks in practice have structure that can be exploited algorithmically. Specifically, common computer network topologies allow a routing path to be uniquely defined by the sender and the receiver, which simplifies algorithm design and analysis. This paper focuses on the symmetric star and the symmetric tree topologies, which are topologies of immense practical interest as they respectively manifest in rack-scale clusters and cloud-based datacenters. The asymmetric star topology is also of great interest for IoT applications, as mobile devices often have different transmitting and receiving capabilities. 

\subsection{Our results}
Our algorithmic results are summarized as follows. 
\begin{table}[h]
	\begin{tabular}{c|c|c|c}
		\hline
		Operator &  Topology & Bandwidth & Optimality \\
		\hline
		set intersection & tree & arbitrary & $O(\log |V| \log N)$ \\
		\hline
		cartesian product & tree & arbitrary & $O(|V|)$ \\
		\hline
		binary join & star & arbitrary & $O(\log |V| \log N)$ \\
		\hline
	\end{tabular}
	\caption{Summary of results.}
\end{table}

For set intersection, the core technique we used is randomized hashing, but designing a family of hash functions to achieve a balanced load is nontrivial. More specifically, each hash function $f: v \to U$ identifies a source node $v$ and a set of designated destination nodes $U = \{u_1, u_2, \cdots, u_k\}$, such that a data is transmitted from $v$ to $u_i \in U$ with some predefined probability $p_i$. The values of $p_i$'s are determined by the initial data cardinality as well as the tree structure.

For square Cartesian product, the hardness comes from the lower bound side which is built on the counting argument. More specifically, we introduce the notion of ``cover'' of compute ndoes in the tree topology such that each cover derives a easier (at least not harder) problem of computing the carteisan product. In this way, the lower bound for each derived problem is also a lower bound for the original one. On the upper bound side, we design a simple one-round routing strategy to achieve the optimal soluition by a factor of $O(|V|)$. Then, we show an improved algorithm to decrease this gap from $O(|V|)$ to $O(1)$. (To be done.)

For binary join, we only investigate the star topology.  Different from set intersection, whose result is at most as large as the input size, a binary join can produce at most quadratic number of results. Previous works in the MPC model~\cite{beame:skew, hu2019output} demonstrate that both the input size and output size characterize the difficulty of a binary join in the distributed computation, and the additional lower bound usually follows a counting argument, where each join result must be produced by some node. Note that in a star topology, edges can be uniquely identified by the compute node at the end. This minimal computation task allocated to each node implies a lower bound of the amount of data arriving at it, i.e., the load on the unique edge incident to it. That's how we transform the counting argument on nodes to the lower bound on the load of edges in a star. On the upper bound, if all the frequencies of join keys are known in advance, we are able to show a deterministic algorithm to achieve the optimal load asymptotically. 

Except the symmetric network, we also investigate the asymmetric network with star topology for set intersection. By combining two simple cases, sending-free star and receiving-free star, we are able to tackle the general asymmetric star under arbitrary bandwidths.


==> join.tex <==
\section{Join}

In the join problem, we are given two relations $R, S$ and the goal is to compute the result of the equi-join $R \Join S$,
such that the output pairs are distributed among the compute nodes by the end of the algorithm. Without any loss of generality, we will assume that the relations are binary; let $\dom$ denote the domain of join attribute.
%
We consider the join for the case of a symmetric star topology under the edge-capacitated model, where the cost function is $f_e(x) = x/w_e$. 

Given an initial distribution $\dstr$ of the data across the compute nodes, we denote
by $R^\dstr_v$, $S^\dstr_v$ the tuples from $R$ and $S$ respectively in node $v$. 
Moreover, denote by $R^\dstr_v(a)$ the tuples from $R$ with join value $a$ and $S^\dstr_v(b)$ the tuples from $S$ with join value $b$, in node $v$. There is $R^\dstr_v = \bigcup_{a \in \mathbf{dom}} R^\dstr_v(a)$ and $S^\dstr_v = \bigcup_{b \in \mathbf{dom}} S^\dstr_v(b)$. Let $N^\dstr_v = |R^\dstr_v| + |S^\dstr_v|$, and $N^\dstr = \sum_v N_v = |R| + |S|$. Whenever the context is clear, we will drop the superscript $\dstr$ from the notation.  For simplicity, assume $|R| \le |S|$. 

Let $\copt$ be the optimal cost (measured in tuples) of any algorithm that knows the initial data distribution.
 
\subsection{Lower Bound on Star Topology}
We consider this problem when the underlying topology is a symmetric star. Let $\copt$ be the capacity cost of any algorithm correctly computing $R \Join S$.  As a general case of both set-intersection and Cartesian product, we first have the following lower bound:

\begin{lemma}
	\label{lem:lb-join-star-1}
	The following lower bound holds:
	\[\copt \ge \max_{v \in V_C} \frac{1}{w_v} \cdot  \min\{|R|, N_v,  N - N_v\}\]
\end{lemma}

\begin{proof}
	Consider a compute node $v \in V_C$ that holds $R_v, S_v$. Suppose that $\copt < |R_v|/w_v$. Then, at least one tuple in $R_v$ does not leave node $v$. In this case, in order to guarantee correctness, all data in $S$ must be sent to node $v$, hence,
	$\copt \geq (|S| - |S_v|)/w_v$. Thus, $w_v \cdot \copt \geq \min \{ |R_v|, |S| - |S_v| \}$.
	
	Using a symmetric argument, $w_v \cdot \copt \geq \min \{ |S_v|, |R| - |R_v| \}$. Summing up the two inequalities, we obtain the desired result.
\end{proof} 

Define a sub-instance with data initial distribution $\dstr'$ as below:
\begin{equation*}
	\begin{aligned}
		R^{\dstr'}_v = R^{\dstr}_v,\\
	\end{aligned}\\ \hspace{2em}
	\begin{aligned}
		S^{\dstr'}_v = \begin{cases}
			\emptyset, & \textrm{if } N_v > |R| \\ 
			S^{\dstr}_v, & \textrm{otherwise} 
		\end{cases}
	\end{aligned}
\end{equation*}
We use $R'_v, S'_v$ as short for $R^{\dstr'}_v, S^{\dstr'}_v$. Let $N'_v = |R'_v| + |S'_v|$. Moreover, $|R'| = \sum_v |R'_v|$, $|S'| = \sum_v |S'_v|$ and $N' = \sum_v N'_v = |R'| + |S'|$.


\begin{lemma}
	\label{lem:lb-join-star-2}
	If $\max_u N_u < |S|$, then $\copt \ge N'/\sum_v w_v$.
\end{lemma}


\begin{proof}
	%%We will prove that this is exactly the lower bound of computing $R' \Join S'$. 
	Under the condition that $\max_u N_u < |S|$, the lower bound from Lemma~\ref{lem:lb-join-star-1} can be rewritten as
	\begin{align*}
	\copt \cdot w_v \ge  \min\{|R|, N_v\} \ge N_v'
	\end{align*}
	for any $v \in V_C$. The rationale behinds the inequality is implied by the definition of $\dstr'$. 
	Summing over all nodes, there is $\sum_v \copt \cdot w_v \ge \sum_v N'_v$, i.e.,  $\copt \ge N'/\sum_v w_v$.
\end{proof}

\subsection{Set Intersection Revisited}
\label{sec:heavy-hitter}
Set intersection is a specical case of join where each join key appears at most once in either relation. In this section, we specify the largest possible frequencies for which the distribution of the join keys will not be influenced by skew. Since the initial data cardinality distribution is given, the skew is defined with resepct to the distribution as well. If there exists some node $v \in V_C$ with $N_v \ge |S|$, then there is no skewness under this distribution. It remains to consider the case that $\max_u N_u < |S|$. 

Note that Algorithm~\ref{alg:set-intersection-star} achieves the lower bound of capacity cost on every edge, by using hash functions depending on the inital data distribution. Here we define a different hash function family by setting $h'_v$ proportional to the capacity cost, i.e. $h'_v = w_v/\sum_v w_v$ for each compute node $v \in V_C$.  %%Note that invoking hash partitioning on the subinstance $\dstr'$ by using $h'$ achieves the capacity cost $O(N'/\sum_v w_v)$ with high probability, which is optimal implied by Lemma~\ref{lem:lb-join-star-2}.


\begin{lemma}
	\label{lem:hashing-2}
	Let $G$ be a symmetric star topology. Suppose that each join key of $R \Join S$ appears in at most $\log |V| \cdot (|R| + |S|)/|V|$ tuples in each relation. Then there is an algorithm correctly computing the binary join with (tuple) cost $\widetilde{O}(C)$ with high probability, where 
	\[C = \frac{|R|+|S|}{\sum_v w_v} + \max_{v} \frac{N_v}{w_v}.\]
\end{lemma}

\begin{proof}
	It suffices to show that if all data are sitting at the router, then the capacity cost is $\widetilde{O}((|R| + |S|)/\sum_v w_v)$. We prove the correctness in two steps. The first is a standard result from the hashing:  suppose that each join key of $R \Join S$ appears in at most $(|R| + |S|) \cdot \min_v w_v/\sum_v w_v$ tuples in either relation, then with high probability the maximum capacity cost is $\widetilde{O}((|R| + |S|)/\sum_v w_v)$. %%More details can be found at Appendix~\ref{appendix:hashing}.
	
	 Moreover, observe that for any set of $\{w_1, w_2, \cdots, w_m\}$ for $w_i \ge 0$, there is $\sum_{j: w_j \ge W/2m \log m} w_j \ge W/\log m$ where $W = \sum_{i=1}^m w_i$. The argument is as follows. For simplicity, assume $w_1 \le w_2 \le \cdots \le w_m$. Find the index $i$ such that $w_i < W/2m \log m \le w_{i+1}$. By contradiction, assume $\sum_{j=i+1}^m w_j < W/\log m$.  Under this circumstances, the value of $w_i$ is at least
	$w_i \ge \frac{1}{i} \cdot \sum_{j =1}^i w_j \ge \frac{1}{m} \cdot (W  - W/\log m ) \ge \frac{W}{2m}$,
	coming to a contradiction.
	
	By invoking the hash join on the compute nodes if the incident edge has capacity at least $w_v \ge W/2|V| \log |V|$, we can obtain the desired result.
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Packing Cartesian Products}
\label{sec:pack-cp}

We define here a protocol that will be a component for the main join algorithm.
The goal is to compute a set of cartesian products $R(a) \times S(a)$, where $a \in A$. 
We initially assume that $|R(a)| = |S(a)|$ for every $a \in A$, and then show how to remove this constraint for general case.
Also, let $N(a) = |R(a)| + |S(a)|$.

\paragraph{Example} Consider an easy case where all $N(a)$'s are equal. The join size is exactly $N \cdot N(a)$. The optimal capacity cost is captured by the following formula:
\[\sum_v (L \cdot w_v) \cdot \min\{L \cdot w_v, N(a)\} \ge N \cdot N(a)\]
Note that for node $v$, the number of tuples it received is at most $L \cdot w_v$. Hence, the maximum number of join results that can be produced on $v$ is $N(a) \cdot L w_v$  if $Lw_v > N(a)$, and $L^2w_v^2$ otherwise. Denote the minimizer as $L^*(N(a), N, V_C)$.

The routing strategy is also implied by the formula directly. We decribe a recursive procedure {\sc PackEQCP}$(A, n, L, V)$ in Algorithm~\ref{alg:pack-eqcp} and the original problem can be solved by just calling {\sc PackEQCP}$(A, N(a), L^*(N(a), N, V_C), V_C)$.

\begin{algorithm}[h]
	\caption{{\sc PackEQCP}$(A, n, L, V)$}
	\label{alg:pack-eqcp}

	Pick an arbitrary join key $a$\;
	$j \gets \arg \max_{v \in V} w_v$\;
	\If{$L \cdot w_j < n$}{
		Send all tuples in $R(a), S(a)$ to node $j$\;
		$w_j \gets w_j - n/L$\;
	}
	\Else{
		Find a subset of nodes $V' \subseteq V$ such that $n^2/2L^2 \le \sum_{i \in V} w^2_i < n^2/L^2$\;
		$V \gets V - V'$\;
	}
	{\sc PackEQCP}$(A - \{a\}, n, L, V)$\;
\end{algorithm}

Now we consider the case where $N(a)$'s can be different but $|R(a)| = |S(a)|$ still holds for each join key $a$. Sort all the keys by the $N(a)$ and relabel them as $a_1, a_2, \cdots, a_k$. Sort all the compute nodes in $V_C$ by the capacities and relabel them as $v_1, v_2, \cdots, v_n$. For short, use $N_i$ to denote $N(a_i)$ and $w_i$ to denote $w_{v_i}$. On the $N = \{N_1, N_2, \cdots, N_k\}$ and $W = \{w_1, w_2, \cdots, w_n\}$, we introduce a recursive procedure {\sc PackCP}$(k,n)$ defined as below:

\paragraph{Base Case} (1) {\sc PackCP}$(k,n) = 0$ if $k = 0$; (2) {\sc PackCP}$(k,n) = + \infty$ if $k \neq 0$ and $n = 0$.

\paragraph{General Case} {\sc PackCP}$(k,n) = $
\begin{align*}
 \min \big\{ & \min_{i \in [k-1]} \max\{\sum_{j=i}^k \frac{N_j}{w_n}, \textrm{{\sc PackCP}}(i-1, n-1) \},	\min_{i \in [n-1]} \max\{\sqrt{\frac{N^2_k}{\sum_{j=i}^n w^2_j}}, \textrm{{\sc PackCP}}(k-1, i-1\}) \} \big \}
\end{align*}

It can be easily verified that Algorithm~\ref{alg:pack-eqcp} is a special case of {\sc PackCP}$(k,n)$. However, it is not possible to obtain a clean form of {\sc PackCP}$(k,n)$ in general. The following Lemma guarantees that {\sc PackCP}$(k,n)$ returns an optimal routing strategy asymptotically and the proof is given in Appendix~\ref{appendix:optimality-packcp}.

\begin{lemma}
	\label{lem:optimality-packcp}
	The {\sc PackCP}$(k,n)$ returns an optimal (within a constant factor) capacity cost.
\end{lemma}

 As long as the statistics of $N$ and $W$ are known by all nodes, the value of {\sc PackCP}$(k,n)$ can be computed locally and the routing strategy is implied as follows. When the minimum value is achieved on the first term with specific value $i^*$, then all tuples of $R(a), S(a)$ with $a \in \{a_{i^*}, a_{i^* +1}, \cdots, a_k\}$ are sent to node $v_n$; and recursively route data by {\sc PackCP}$(i^*-1, n-1)$. When the minimum value is achieved on the second term with specific value $i*$, then run wHC algorithm for computing $R(a_k) \times S(a_k)$ on the compute nodes $\{v_{i^*}, v_{i^*+1}, \cdots, v_n\}$; and recursively route data by  {\sc PackCP}$(k-1,i^*-1)$.

\begin{proof}
	We prove this result under the assumption that each join key has equal input size in two relations through step 1-4, and then extend it to general cases. In the following, ``asympoticial' always mean "within a constant factor". Our proof builds on the following observation. Assume each compute node $v \in V_C$ has a budget $x_v > 0$ in computing the Cartesian product $R \times S$ where $|R| = |S|= N$.  Moreover, all the data are sitting at the router. There exists a routing strategy without exceeding the budget by a constant factor if $\sum_{v \in V_C} x^2_v \ge N^2$.
	By setting $\frac{N}{\sqrt{\sum_v w^2_v}} \cdot w_v = x_v$ for each $v \in V_C$, running Algorithm~\ref{alg:balanced-packing} yields the result directly.
	
	We introduce some notation and terminology first. Consider any feasible solution $sol$ of packing the given Cartesian products. For $sol$, we constrcut a {\em computation hypergraph} denoted as $G_{sol}$ from $sol$: introduce a vertex for each join key $a$ and an edge for each compute node $v \in V_C$ such that $a \in v$ if node $v$ participates in partial or whole computation of the Cartesian product of $a$.  A key is {\em unique} if it only appears in one node and {\em joint} otherwise. A node is {\em singleton} if it contains only one key and {\em non-singleton} otherwise. 
	
	\paragraph{Step 1}	There is an asymptotically optimal solution such that $|R(v,a)| = |S(v,a)|$ holds for each join key $a$ and each compute node $v \in V_C$. 
	
	\medskip
	We show that any optimal solution can be transformed into an asymptotical one whose derived computation hypergraph is berge-acyclic. After data shuffling, denote $R(v,a), S(v,a)$ as the set of $R$-tuples and $S$-tuples with key $a$ locating at $v$. Observe that in the optimal solution there is $|R(v,a)| = |S(v,a)|$ for any $a \in $ and $v \in V_C$. Proof by contradiction, assume there exists some key $a$ and node $v \in V_C$ with $|R(v,a)| \neq |S(v,a)|$. Only consider such a join key $a$, where each server $v \in V_C$ has a budget $|R(v,a)| + |S(v,a)|$. We construct an solution such that (1) tuples with join key $a'$ if $a' \neq a$ are routed as the same as $opt$; (2) tuples with join key $a$ are routed implied by Lemma~\ref{lem:budget}. We apply this procedure for each join key $a$ if there exists compute node $v$ with $|R(v,a)| \neq |S(v,a)|$. Denote the resulted solution as $opt'$. Note that the capacity cost of $opt'$ is increased by at most a constant factor from $opt$. More importantly, there is $|R(v,a)| = |S(v,a)|$ for each join key $a \in A$ and each compute node $v \in V_C$.
	
	\paragraph{Step 2} There is an asymptotically optimal solution whose derived computation hypergraph is berge-acyclic.
	
	\medskip
	
	Denote the optimal solution identified from the last step as $opt$. For simplicity, denote $|R(v,a)| = |S(v,a)| = N(v,a)$. It is known that a hypergraph is berge-acyclic if and only if its incidence graph is acyclic.  By contradiction, assume $H_{opt}$ is not berge-acyclic, i.e., there exists a cycle $a_1v_1a_2v_2a_3v_3\cdots a_nv_na_1$, where $v_i \cap v_{(i+1)\mod n} = \{a_i\}$ for $i \in\{1,2,\cdots,n\}$. Without loss of generality, assume $\sum_i N(a_i, v_i) \ge \sum_i N(a_{(i+1)\mod n}, v_i)$. Define $\Delta = \min\{N(a_2, v_1), N(a_3, v_2), \cdots, N(a_1, v_n)\}$,  where the minimum value is achieved on $N(a_{(i+1) \mod n}, v_i)$. Shifting $\Delta$ tuples with key $a_{(i+1) \mod n}$ from node $v_{i}$ to node $v_{(i+1)\mod n}$ will yields a better (at least not worse) solution since 
	\begin{align*}
	& \sum_i (N(a_i, v_i) + \Delta)^2 + (N(a_{i+1}, v_i) - \Delta)^2 \ge \sum_i N(a_i, v_i)^2 + N(a_{i+1}, v_i)^2 + 2 \Delta \cdot (\sum_i N(a_i, v_i)- \sum_i N(a_{i+1}, v_i)) + 2 \cdot \sum_i \Delta^2
	\end{align*}
	In this solution, node $v_i$ only contains key $a_i$ and key $a_{i+1}$ only exists in node $v_{i+1}$. Then $v_i$ and $a_{i+1}$ can be removed from this cycle. Apply this procedure recursively, we can remove all edges except at most two, thus breaking this cycle.  Note that in this transformation, the number of tuples locating at each node stays the same, thus the resulted solution is also optimal. 
	
	
	\paragraph{Step 3} There is an asymptotically optimal solution which uses at most 2 copies of the original compute nodes such that each node either is a singleton or contains only unique keys. 
	
	\medskip
	
	Consider the optimal solution identified by the last step as $opt$. In a berge-acyclic hypergraph, every pair of nodes share no more than one common keys. 
	
	We transform $H_{opt}$ into a new solution $H_{opt'}$ as follows. If there is a singleton node $v \in V_C$, then remove it from $H_{opt}$ and add it to $H_{opt'}$. Otherwise, there exists one node containing only one joint key due to the property of berge-acyclic hypergraph. Split this node into two copies, one including all unique keys and the other including the joint key. Remove this node from $H_{opt}$ and add the two copies to $H_{opt'}$.  After applying this step recursively, $H_{opt}$ will become an empty hypergraph and each node has at most two copies in $H_{opt'}$. Observe that each key appears in at most one non-singleton node in $H_{opt'}$. By contradiction, assume key $a$ appears in nodes $v, v'$ both of which contain more than one key.  With loss of generality, assume node $v$ is added to $H_{opt'}$ before $v'$. By the rule above, $v$ is added as a set of unique keys, which is a contradiction to the fact that $a$ is a joint key. 
	
	Then, we transform $H_{opt'}$ into a new solution $H_{opt''}$ as follows. Consider an arbitrary key $a$ appearing in a non-singleton node $v$. If $N(v,a) \ge \sum_{v': v' \neq v} N(v', a)$, then merge all singletons containing $a$ with $v$ and remove these singletons. Otherwise, distribute all tuples of $R(v,a)$, $S(v,a)$ to all singletons containing $a$ proportionally and remove $a$ from node $v$. After this step, each non-singleton node only contains unique keys. Moreover, in the transformation, the number of tuples locating at each node is increased by at most a factor of $2$. Thus we have obtain an asymptotically optimal solution as desired. 
	
	
	\paragraph{Step 4} {\sc PackCP} returns an asymptotically optimal solution.
	
	\medskip
	
	By the analysis above, we need to consider solutions where each node computes the full Cartesian product of multiple keys or just the partial Cartesian product of one key. Denote the optimal solution identified by the last step as $opt$ with capacity $C$. 
	
	If $C \cdot w_n \le N_k$, $a_k$ must be a joint key in $H_{opt}$. Assume the indexes of singletons that participate in the computation of $R(a_k) \times S(a_k)$ as $V_k$. We claim that $V_k$ is a suffix of $\{v_1,v_2, \cdots,v_n\}$. Proof by contradiction, assume that $j$ is the largest index not included by $V_k$. Pick the set of smallest indexes in $V_k$ as $V'$ such that $\frac{1}{2} w^2_j \le \sum_{i \in V'} w_i^2 < 2 w_j^2$. The computation performed on node $v_j$ can always be covered by nodes in $V'$, thus exchanging the allocation between $v_j$ and $V'$ will not violate the capacity constraints. The property that $V_k$ is a suffix of $\{v_1,v_2, \cdots,v_n\}$ is characterized by the recurrence formula of {\sc PackCP}.
	
	Otherwise, $C \cdot w_n > N_k$. More specifically, find an index $i$ such that $N_{j=i}^k \le C \cdot w_n < N_{j=i-1}^k$. We claim that all keys in $\{a_i, a_{i+1}, \cdots, a_k\}$ are allocated to $v_n$ as unique keys. Proof by contradiction, assume that $j \in \{i, i+1, \cdots, k\}$ is the largest index not allocated to $v_n$. Pick the set of keys on $v_n$ as $A'$ such that $\frac{1}{2} N_j \le \sum_{a \in A'} N(a) < N_j$. If $a_j$ is allocated to $v_h$ as a unique key, then exchange $A'$ with $a_j$.
	If $a_j$ is allocated to a subset of nodes $V_j$ as a joint key, then the computation performed for keys in $A'$ on nodes $v_n$ can always be covered by that for key $a_j$ on nodes in $V_j$. In either way, the exchange will not violate the capacity constraint. The fact that the join keys allocated for $v_n$ is a suffix of $\{a_1, a_2, \cdots, a_k\}$ is also characterized by the recurrence formula of {\sc PackCP}.
	
	\medskip 
	Last but not least, we extend the result to a general instance $\mathbf{R}$ where there exists some join key $a$ with $|R(a)| \neq |S(a)|$. Denote the optimal solution of computing $\mathbf{R}$ as $opt$ with cost $\copt$. Recall that $R(v,a), S(v,a)$ are the set of $R$-tuples and $S$-tuples with key $a$ locating at node $v$. Moreover, let $N(v,a)$ be the size of tuples with key $a$ loaded by node $v$. W.l.o.g. assume $|R(a)| < |S(a)|$. Observe that there exists an optimal solution such that (1) if $N(v,a) < 2 |R(a)|$, then $|R(v,a)| = |S(v,a)|$; (2) otherwise, $|R(v,a)|= |R(a)|$ and $|S(v,a)| = N(v,a) - |R(a)|$. This can be easily proved by the counting argument, similar to step 1. 
	
	
	We transform $\mathbf{R}$ into a new instance $\mathbf{R'}$ as follows. For a join key $a$ with $|R(a)| < |S(a)|$, divide the set $S(a)$ into $|S(a)|/|R(a)|$ disjoint subsets, each of size $|R(a)|$. Then computing the Cartesian product of size $|R(a)| \times |S(a)|$ is transformed into $|S(a)|/|R(a)|$ Cartesian products of size $|R(a)| \times |R(a)|$. The case with $|R(a)| > |S(a)|$ is handled symmetrically. Denote the capacity cost of computing $\mathbf{R'}$ by {\sc PackCP} as $C'_{opt}$. Note that the optimal solution $opt$ is also a candidate solution for $\mathbf{R'}$ with capacity cost at most $2 \copt$. Hence $\copt' \le 2 \copt$. In this way, we obtain an asymptotically optimal solution for $\mathbf{R}$ eventually.
\end{proof}



\subsection{Algorithm on Symmetric Star}
We now present an algorithm that matches the two lower bounds of the above section.

\begin{algorithm}[h]
	\caption{{\sc StarJoin}$(G,\dstr)$}
	\label{alg:join-star}

	\If{$\max_u N_u \ge |S|$}{
		All nodes send their data to $\arg \max_u N_u$\;
	}
	\Else{
		$V_\alpha = \{v \in V_C \mid \min\{N_v, N- N_v\} < |R|\}$\;
		$V_\beta = V_C - V_\alpha$\;
		All nodes send their $R$-tuples to nodes in $V_\beta$\;
		$R' \gets R$, $S' \gets S - \bigcup_{v: N_v > |R|} S_v$\;
		$H \gets \{a \in \mathbf{dom}: N'(a) \ge N'/|V| \cdot \log |V|\}$\;
		Apply hash join to compute $\sigma_{a \notin H} R' \Join \sigma_{a \notin H} S'$\;
		Apply {\sc PackCP} to compute $\bigcup_{a \in H} R'(a) \times S'(a)$\;
	}
\end{algorithm}

In Algorithm~\ref{alg:join-star}, the capacity cost of the first case (line 1-2) is matched by Lemma~\ref{lem:lb-join-star-1}. In the second case, then each join key $a$ is defined as {\em heavy} if its degree in either $R'$ or $S'$ is greater than $N' \cdot \log |V|/\sum_v w_v$ and {\em light} otherwise. Note that there are at most $|V|$ heavy join keys. For tuples with light join keys, just invoke the hash join. For tuples with heavy join keys, invoke the packing algorithm to compute a union of Cartesian products. The capacity costs of line 6 and line 9-10 are matched by Lemma~\ref{lem:lb-join-star-2} and Lemma~\ref{lem:optimality-packcp}. Hence the algorithm is asymptotically optimal.


